Replay Attacks and Defenses Against Cross-shard Consensus in Sharded Distributed Ledgers

We present a family of replay attacks against sharded distributed ledgers, that target cross-shard consensus protocols, such as the recently proposed Chainspace and Omniledger. They allow an attacker, with network access only, to double-spend or lock resources with minimal efforts. The attacker can act independently without colluding with any nodes, and succeed even if all nodes are honest; most of the attacks can also exhibit themselves as faults under periods of asynchrony. These attacks are effective against both shard-led and client-led cross-shard consensus approaches. Finally, we present Byzcuit - a new cross-shard consensus protocol that is immune to those attacks. We implement a prototype of Byzcuit and evaluate it on a real cloud-based testbed, showing that our defenses impact performance minimally, and overall performance surpasses previous works.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	main.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

==> appendices/proofs.tex <==
% =========
% Proofs 
% =========
%\section{Proofs of \Cref{th:secure-phase-1} and \Cref{th:secure-phase-2}} \label{sec:proofs}
\section{Security against Replay Attacks} \label{sec:proofs}
The security proofs of \Cref{th:secure-phase-1} and \Cref{th:secure-phase-2} of \Cref{sec:security} rely on \Cref{le:secure-phase-1}.

%
\begin{lemma} \label{le:secure-phase-1}
Under Honest Shard assumption, no \attacker can obtain \prerecorded messages containing a fresh transaction sequence number $s_T$.
\end{lemma}
\begin{proof}
The core idea protecting \sysname from these replay attacks is that the \attacker can only obtain \prerecorded messages associated with old transaction sequence numbers $s_T$. The transaction sequence number $s_T$ is fresh only if it is at least equal the maximum of the sequence number of all input and dummy objects of the transaction $T$. Shards update every input and dummy object sequence number upon aborting transactions in such a way that sequence numbers only increase. That is, after emitting \preacceptts or \preabortts, either the sequence number of all input and dummy objects of $T$ are updated to a value bigger than $s_T$ (in case of \preabortts), or the objects are inactivated which prevents any successive transaction to use them as input (in case of \preacceptts).
It is therefore impossible for the adversary to hold a \prerecorded message for a fresh $s_T$ since the only \prerecorded messages that the adversary can obtain contain sequence numbers smaller than $s_T$.
\end{proof}
%


% =========
%\subsection{Proof of \Cref{th:secure-phase-1}}\label{sec:proof-th1}
\subsection{Proof of Theorem 1}\label{sec:proof-th1}
%
\begin{prooftheorem}
Under Honest Shard assumption, \sysname ignores \acceptts and \abortts messages issued from replayed \preacceptts and \preabortts.
\end{prooftheorem}
\begin{proof}
\Cref{fig:byzcuit-fsm} shows that once \sysname locks objects for a particular pair $(T,s_T)$, the protocol can only progress toward \acceptts or \abortts; \ie shards can either accept or abort the transaction $T$. The \attacker aims to trick one or more shards to incorrectly accept or abort $T$ by injecting \prerecorded messages during the first phase of \sysname; we show that the \attacker fails in every possible scenario. 

Suppose transaction $T$ should abort (the TM outputs \abortts), but the \attacker tries to trick some shards to accept the transaction. \Cref{fig:byzcuit-fsm} shows that the \attacker can only succeed the attack if they gather \acceptts containing a fresh transaction sequence number $s_T$. Lemma~\ref{le:secure-phase-1} states that no \attacker can obtain \prerecorded messages over a fresh transaction sequence number $s_T$; therefore the only messages available to the adversary at this point of the protocol are (at most) $n-1$ \preacceptts and (at most) $n$ \abortts, where $n$ is the number of concerned shards. This is not enough to form an \acceptts message with a fresh transaction sequence number $s_T$ (which is composed of $n$ \preacceptts); therefore the \attacker cannot trick any shard to accept the transaction.

Suppose transaction $T$ should be accepted (the TM outputs \acceptts with a fresh $S_T$), but the \attacker tries to trick some shards to abort the transaction. \Cref{fig:byzcuit-fsm} show that \sysname does not require a fresh transaction sequence number $s_T$ to abort transactions (the freshness of $s_T$ is only enforced upon accepting a transaction); but shards locked the input and dummy objects of the transaction for the pair $(T,s_T)$ (with fresh $s_T$), so the attacker needs to gather \abortts containing the same transaction sequence number $s_T$ locked by shards.  Lemma~\ref{le:secure-phase-1} shows that the \attacker cannot obtain \prerecorded messages over fresh $s_T$; therefore the only messages available to the adversary containing the (fresh) $s_T$ locked by shards at this point of the protocol are $n$ \preacceptts. This is not enough to form an \abortts message (which is composed of at least one \preabortts); therefore the \attacker cannot trick any shard to abort the transaction.
\end{proof}
%



% =========
%\subsection{Proof of \Cref{th:secure-phase-2}}\label{sec:proof-th2}
\subsection{Proof of Theorem 2}\label{sec:proof-th2}

%
\begin{prooftheorem}
Under Honest Shard assumption, \sysname ignores replayed \acceptts and \abortts messages.
\end{prooftheorem}
\begin{proof}
\Cref{fig:byzcuit-fsm} shows that shards only act upon \acceptts and \abortts messages if they have the pair $(T,s_T)$ saved in their local cache\footnote{Contrarily to \sbac and \atomix, all \sysname shards have the pair $(T,s_T)$ in their local cache after as they all participate to the first phase of the protocol.}. Shards save a pair $(T,s_T)$ in their local cache upon emitting \preacceptts or \preabortts, and delete it at the end of the protocol; therefore the only attack windows where the adversary can replay \acceptts and \abortts messages is while the transaction $T$ (associated with $s_T$) is being processed by the second phase of \sysname. This forces the attacker to operates under the same conditions as \Cref{th:secure-phase-1}, which is proven secure in \Cref{sec:proof-th1}.
\end{proof}
%



==> sections/old_text.tex <==
\Cref{fig:sbac-mitigation-fsm} shows that upon receiving a new transaction, shards lock input objects for a given transaction and sequence number $s$, and send \textsf{pre-accept}($T,s$) or \textsf{pre-abort}($T,s$) to the Transaction Manager (see \Cref{fig:lsbac}). 



===

Shards sequence the transaction and send \textsf{pre-accept}($T$) or \textsf{pre-abort}($T$) messages to the TM; similarly to \sbac, shards lock the input objects upon emitting \textsf{pre-accept}($T$). The TM then aggregates and reflects these messages to all shards involved in the transaction by sending \textsf{accept}($T$) or \textsf{abort}($T$). Shards interpret the message; they unlock the objects if they receive \textsf{abort}($T$), or (permanently) invalidate them if they receive \textsf{accept}($T$). 
It is then sufficient that one shard notify the outcome to the client.



===




% =========
%\subsection{Security against Replay Attacks} \label{sec:lsbac:security}
%We show how \lsbac mitigates the replay attacks against \sbac described in Sections~ \ref{chainspace}~and~\ref{omniledger}.

%\paragraph{Security of the first phase of \sysname} An \attacker may try to replay \preacceptt and \preabortt messages during the first phase of the atomic commit protocol, as described in \Cref{chainspace-attack-1} and \ref{omniledger-attack-1}. \Cref{th:sbac-mitigation} shows how \sysname leverages the object sequence numbers introduced in \Cref{sec:lsbac:design} to mitigate those attacks. We divide \Cref{th:sbac-mitigation} into a lemma and a corollary to prove it; we recall \emph{consistency} in the context of \sbac (\Cref{th:sbac-consistency}) which also applies to \sysname.

%\begin{theorem}\label{th:sbac-consistency}
%(\sbac~\cite{chainspace}) Consistency: Under the `honest shards' threat model, no two conflicting transactions, namely transactions sharing the same input will be committed. Furthermore, a sequential executions for all transactions exists.
%\end{theorem}

%\begin{corollary}\label{co:sbac-original-same-output}
%If all shards ignore replayed messages, \sysname terminates successfully.
%\end{corollary}
%\begin{proof}
%If all shards follow the protocol and there is no adversary (\ie there are no replayed messages), consistency follows from \Cref{th:sbac-consistency} and thus \sysname terminates successfully.\footnote{\Cref{th:sbac-consistency} implies successful termination despite a number of byzantine nodes, but our attacks work also in a setting where all nodes are honest (see \Cref{attack-overview}).}
%\end{proof}

%\begin{lemma}\label{le:sbac-ignore-bad-messages}
%Let's assume that each shard follows the FSM shown in %\Cref{fig:sbac-mitigation-fsm}. Shards ignore replayed message.
%\end{lemma}
%\begin{proof}
%\Cref{fig:sbac-mitigation-fsm} shows that shards lock objects for a given transaction and sequence number $s$. Shards only emit \textsf{pre-accept}($T,s$) or \textsf{pre-abort}($T,s$) with a fresh sequence number $s$ (\ie the sequence number $s$ is never re-used); regardless whether they decide to commit or abort, the sequence number associated with every object in the transaction is updated in such a way that it only increases. Therefore, shards detect replayed messages because they contains passed sequence numbers, and thus ignore the message. During the second phase of the protocol, shards ignore \textsf{pre-accept}($T,s$) and \textsf{pre-abort}($T,s$) messages if they did not previously locked the objects in the transaction $T$ for that given sequence number $s$. Shards verifies that $s$ is well formed before emitting an \textsf{accept}($T,s$) message; thus, recalling that all messages are signed (and thus can only be generated by shards), no shard can be fooled to act upon replayed \textsf{pre-accept}($T,s$) or \textsf{pre-abort}($T,s$) messages.
%\end{proof}

%\begin{theorem} \label{th:sbac-mitigation}
%Let's assume that each shard follows the FSM shown in %\Cref{fig:sbac-mitigation-fsm}. The attacks described in \Cref{chainspace-attack-1} %(and \Cref{tab:sbac-attack}) cannot happen.
%\end{theorem}
%\begin{proof}
%Corollary~\ref{co:sbac-original-same-output} states that if all shards ignore replayed \textsf{pre-accept}($T,s$) and \textsf{pre-abort}($T,s$) messages, the protocol successfully terminates; and Lemma~\ref{le:sbac-ignore-bad-messages} states that shards ignore those replayed messages if shards follow he FSM shown in \Cref{fig:sbac-mitigation-fsm}. Therefore, \sysname executes successfully if shards follow the FSM shown in \Cref{fig:sbac-mitigation-fsm}.
%\end{proof}

%The above mitigation introduces a new security risk. A malicious user could submit a pair $(T,s)$ such that the sequence number $s$ is just below the overflow value. The sequence number associate with the objects would overflow upon the next updates, and the attack scenarios described in \Cref{chainspace-attack-1} can happen again\footnote{Note that this overflow vulnerability is common to every system relying on nonces chosen by the users, like Byzantine Quorum Systems~\cite{malkhi1998byzantine}.}. To mitigate this issue, smart contracts could define an identity procedure allowing shards to update any object of the contract to an unchanged version of themselves. After the execution of this identity procedure, the object id changes, thus creating a new object with serial number $s'=0$. When shards detect that the serial number of one of their objects approaches the overflow value, they would lock the object and execute this identity procedure.

%\paragraph{Security of the second phase of \sysname} \lsbac is resilient by design to the attacks against the second phase of the atomic commit protocol described in \Cref{chainspace-attack-2} and \Cref{omniledger-attack-2}. The core of these attacks comes from the fact that shards acting only as output shards do not have any information about input objects, and do not communicate with the input shards during the first phase of the protocol. Therefore, they cannot experience the freshness of messages and ensure that they are issued from the same instance of the protocol. \sysname is designed in such a way that there are no shards that act only as output shards (by introducing dummy objects); this avoids the attacks setting described in \Cref{chainspace-attack-2} and \Cref{omniledger-attack-2}, as the attack targets no longer exist.

==> sections/related-works.tex <==
% =========
% Related Works
% =========
\section{Related Works} \label{sec:related-works}
\alberto{Related works on replay attacks, and perhaps other attacks against blockchains.}

==> sections/rscoin.tex <==
% =========
% RSCoin 
% =========
\section{\rscoin} \label{sec:rscoin}
\alberto{@Mustafa, could you handle this section? Check if the replay attack applies to RSCoin as well, and remove this section if it doesn't.}

% =========
\subsection{Summary} \label{sec:rscoin:summary}

% =========
\subsection{Attack} \label{sec:rscoin:attack}

% =========
\subsection{Mitigation} \label{sec:rscoin:mitigation}
